EDoG: Adversarial Edge Detection For Graph Neural Networks

Graph Neural Networks (GNNs) have been widely applied to different tasks such as bioinformatics, drug design, and social networks. However, recent studies have shown that GNNs are vulnerable to adversarial attacks which aim to mislead the node or subgraph classification prediction by adding subtle perturbations. Detecting these attacks is challenging due to the small magnitude of perturbation and the discrete nature of graph data. In this paper, we propose a general adversarial edge detection pipeline EDoG without requiring knowledge of the attack strategies based on graph generation. Specifically, we propose a novel graph generation approach combined with link prediction to detect suspicious adversarial edges. To effectively train the graph generative model, we sample several sub-graphs from the given graph data. We show that since the number of adversarial edges is usually low in practice, with low probability the sampled sub-graphs will contain adversarial edges based on the union bound. In addition, considering the strong attacks which perturb a large number of edges, we propose a set of novel features to perform outlier detection as the preprocessing for our detection. Extensive experimental results on three real-world graph datasets including a private transaction rule dataset from a major company and two types of synthetic graphs with controlled properties show that EDoG can achieve above 0.8 AUC against four state-of-the-art unseen attack strategies without requiring any knowledge about the attack type; and around 0.85 with knowledge of the attack type. EDoG significantly outperforms traditional malicious edge detection baselines. We also show that an adaptive attack with full knowledge of our detection pipeline is difficult to bypass it.

==> discuss.tex <==
\section{Discussion}
\xiaojun{no need for adaptive attacks. If no other discussion, maybe remove this sec.}
\subsection{Adaptive Attacks}
Adaptive attack is a major concern in the study of defense against adversarial machine learning and many works have been shown vulnerable when the attacker knows the defense mechanism\cite{carlini2017magnet}. In this work, the adaptive attack threat facing us is as following: suppose the attacker has full knowledge of our \ensembs pipeline, is he able to add malicious edges which look benign to the system and can fool the GNN? For us, the answer is no because of two reasons.

First, different with many detection pipelines\cite{Meng2017MagNet} on machine learning adversaries which train a static model for detecting various adversarial examples, in this work we will have a different model with respect to different input examples. In particular, we train \ensembs each time we are provided with a (possibly malicious) graph. Therefore, the attacker cannot add malicious edges in order to fool the detection model in use. Each time the graph is changed, the detection model will also change.

Moreover, in \ensemb we propose \graphgs that uses graph generation techniques to detect malicious edges. Adversarial attack against graph generation algorithms is difficult to perform due to its complexity. To the best of our knowledge, there is no existing work on how to attack a graph generation model. Hence, we conclude that our \ensemb system is robust to detect malicious edges even the attacker knows our entire pipeline.

\subsection{Detection vs. Defense}
In this paper we focus on detecting malicious edges in a graph under attack. There are also works aiming to directly defend against the attack and mitigate the effect of malicious edges \cite{zhu2019robust}. The latter approach is more convenient in practice since it directly avoid being attacked by the adversary. However, we would like to argue that our approach is superior in two properties: first, detecting the malicious edge can help identify the attacker. For example, in the case of social network we can find out which user is adding the malicious link. Second, the latter approaches are usually more prone to adversarial attack, since they incorporate the defense mechanism in the model and are therefore easier to be attacked as a whole when the attacker has knowledge of the mechanism.


% \subsection{Graph Sampling Policy}
% \xiaojun{add discussion if we are short of contents.}
